Lambek pregroups are Frobenius spiders in preorders

"Spider" is a nickname of special Frobenius algebras, a fundamental structure from mathematics, physics, and computer science. Pregroups are a fundamental structure from linguistics. Pregroups and spiders have been used together in natural language processing: one for syntax, the other for semantics. It turns out that pregroups themselves can be characterized as pointed spiders in the category of preordered relations, where they naturally arise from grammars. The other way around, preordered spider algebras in general can be characterized as unions of pregroups. This extends the characterization of relational spider algebras as disjoint unions of groups. The compositional framework that emerged with the results suggests new ways to understand and apply the basis structures in machine learning and data analysis.

==> PIC/comonoid.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Mar 25 06:42:11 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.63" x-max="123.75" y-min="-0.62" y-max="25" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(117.5,10)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$=$
%</text>
%<text right-arrow= "head"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,10)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$=$
%</text>
%<ellipse right-arrow= "head"
%	 p3= "(34.06,12.19)"
%	 p2= "(34.06,9.06)"
%	 p1= "(37.19,9.06)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve points= "(40.62,18.12);(40.62,18.12);(40.62,17.5);(40.62,17.5);(40.62,17.5);(40.63,15.62);
%	(40.63,15.62);(40.63,15.62);(36.88,11.87);(36.88,11.87)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(30.62,18.12);(30.62,18.12);(30.62,17.5);(30.62,17.5);(30.62,17.5);(30.63,15.62);
%	(30.63,15.62);(30.63,15.62);(34.38,11.87);(34.38,11.87)"
%	 fill-style= "none"
%	 />
%<ellipse right-arrow= "head"
%	 p3= "(27.81,5.94)"
%	 p2= "(27.81,2.81)"
%	 p1= "(30.94,2.81)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve points= "(5.62,9.38);(5.62,9.38);(10.62,4.38);(10.62,4.38);(10.62,4.38);(9.38,4.38);
%	(9.38,4.38);(9.38,4.38);(10,4.38);(10,4.38)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(24.37,17.5);(24.37,17.5);(24.38,11.25);(24.38,11.25);(24.38,11.25);(24.38,9.37);
%	(24.38,9.37);(24.38,9.37);(28.13,5.62);(28.13,5.62)"
%	 fill-style= "none"
%	 />
%<ellipse right-arrow= "head"
%	 p3= "(2.81,12.19)"
%	 p2= "(2.81,9.06)"
%	 p1= "(5.94,9.06)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<ellipse right-arrow= "head"
%	 p3= "(8.75,6.25)"
%	 p2= "(8.75,3.12)"
%	 p1= "(11.88,3.12)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve points= "(15,17.5);(15,17.5);(15,15);(15,15);(15,15);(15,9.37);
%	(15,9.37);(15,9.37);(11.25,5.62);(11.25,5.62)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(34.38,9.38);(34.38,9.38);(29.38,4.38);(29.38,4.38);(29.38,4.38);(29.38,4.38);
%	(29.38,4.38);(29.38,4.38);(29.38,4.38);(29.38,4.38)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(9.37,17.5);(9.37,17.5);(9.37,16.87);(9.37,16.87);(9.37,16.87);(9.38,15);
%	(9.38,15);(9.38,15);(5.63,11.25);(5.63,11.25)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(-0.63,17.5);(-0.63,17.5);(-0.63,16.87);(-0.63,16.87);(-0.63,16.87);(-0.62,15);
%	(-0.62,15);(-0.62,15);(3.13,11.25);(3.13,11.25)"
%	 fill-style= "none"
%	 />
%<text right-arrow= "head"
%	 text-vert-align= "center-v"
%	 anchor-point= "(88.75,10)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$=$
%</text>
%<ellipse right-arrow= "head"
%	 p3= "(106.56,12.81)"
%	 p2= "(106.56,9.69)"
%	 p1= "(109.69,9.69)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<ellipse right-arrow= "head"
%	 p3= "(100.31,6.56)"
%	 p2= "(100.31,3.44)"
%	 p1= "(103.44,3.44)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve points= "(70.62,10);(70.62,10);(75.62,5);(75.62,5);(75.62,5);(74.38,5);
%	(74.38,5);(74.38,5);(75,5);(75,5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(101.88,3.75);(101.88,3.75);(101.88,0);(101.88,0);(101.88,0);(101.88,-0.62);
%	(101.88,-0.62);(101.88,-0.62);(101.88,0);(101.88,0)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(96.87,18.12);(96.87,18.12);(96.88,11.87);(96.88,11.87);(96.88,11.87);(96.88,10);
%	(96.88,10);(96.88,10);(100.63,6.25);(100.63,6.25)"
%	 fill-style= "none"
%	 />
%<ellipse right-arrow= "head"
%	 p3= "(67.81,12.81)"
%	 p2= "(67.81,9.69)"
%	 p1= "(70.94,9.69)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<ellipse right-arrow= "head"
%	 p3= "(73.75,6.87)"
%	 p2= "(73.75,3.75)"
%	 p1= "(76.88,3.75)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve points= "(80,18.12);(80,18.12);(80,15.62);(80,15.62);(80,15.62);(80,10);
%	(80,10);(80,10);(76.25,6.25);(76.25,6.25)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(75,3.75);(75,3.75);(75,0);(75,0);(75,0);(75,-0.62);
%	(75,-0.62);(75,-0.62);(75,0);(75,0)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(106.88,10);(106.88,10);(101.88,5);(101.88,5);(101.88,5);(101.88,5);
%	(101.88,5);(101.88,5);(101.88,5);(101.88,5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(29.38,3.12);(29.38,3.12);(29.38,0);(29.38,0);(29.38,0);(29.38,-0.62);
%	(29.38,-0.62);(29.38,-0.62);(29.38,0);(29.38,0)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(10,3.12);(10,3.12);(10,0);(10,0);(10,0);(10,-0.62);
%	(10,-0.62);(10,-0.62);(10,0);(10,0)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(123.75,18.12);(123.75,18.12);(123.75,0);(123.75,0);(123.75,0);(123.75,-0.62);
%	(123.75,-0.62);(123.75,-0.62);(123.75,0);(123.75,0)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqone$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(96.25,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqtwo$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(123.75,25)
\rput(117.5,10){$=$}
\rput(20,10){$=$}
\rput{0}(35.62,10.62){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(40.62,18.12)
(40.62,17.5)
(40.63,15.62)(36.88,11.87)
\psline(30.62,18.12)
(30.62,17.5)
(30.63,15.62)(34.38,11.87)
\rput{0}(29.38,4.38){\psellipse[fillstyle=solid](0,0)(1.57,-1.57)}
\psline(5.62,9.38)
(10.62,4.38)
(9.38,4.38)(10,4.38)
\psline(24.37,17.5)
(24.38,11.25)
(24.38,9.37)(28.13,5.62)
\rput{0}(4.38,10.62){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\rput{0}(10.32,4.69){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\psline(15,17.5)
(15,15)
(15,9.37)(11.25,5.62)
\pscustom[]{\psline(34.38,9.38)(29.38,4.38)
\psbezier(29.38,4.38)(29.38,4.38)(29.38,4.38)
\psbezier(29.38,4.38)(29.38,4.38)(29.38,4.38)
}
\psline(9.37,17.5)
(9.37,16.87)
(9.38,15)(5.63,11.25)
\psline(-0.63,17.5)
(-0.63,16.87)
(-0.62,15)(3.13,11.25)
\rput(88.75,10){$=$}
\rput{0}(108.12,11.25){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\rput{0}(101.88,5){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(70.62,10)
(75.62,5)
(74.38,5)(75,5)
\psline(101.88,3.75)
(101.88,0)
(101.88,-0.62)(101.88,0)
\psline(96.87,18.12)
(96.88,11.87)
(96.88,10)(100.63,6.25)
\rput{0}(69.38,11.25){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(75.32,5.31){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(80,18.12)
(80,15.62)
(80,10)(76.25,6.25)
\psline(75,3.75)
(75,0)
(75,-0.62)(75,0)
\pscustom[]{\psline(106.88,10)(101.88,5)
\psbezier(101.88,5)(101.88,5)(101.88,5)
\psbezier(101.88,5)(101.88,5)(101.88,5)
}
\psline(29.38,3.12)
(29.38,0)
(29.38,-0.62)(29.38,0)
\psline(10,3.12)
(10,0)
(10,-0.62)(10,0)
\psline(123.75,18.12)
(123.75,0)
(123.75,-0.62)(123.75,0)
\rput(20,25){$\eqone$}
\rput(96.25,25){$\eqtwo$}
\end{pspicture}


==> PIC/frobspec.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Apr 24 14:28:51 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-1.25" x-max="111.25" y-min="0" y-max="30" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqtwo$
%</text>
%<multicurve fill-style= "none"
%	 points= "(15,20);(15,20);(15,12.5);(15,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,6.25);(10,6.25);(10,0);(10,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0.01,7.5);(0.01,7.5);(0,0);(0,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,12.5);(15,12.5);(11.25,8.75);(11.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0.01,7.5);(0.01,7.5);(3.76,11.25);(3.76,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.26,11.25);(6.26,11.25);(8.76,8.75);(8.76,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,20);(5,20);(4.99,13.75);(4.99,13.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqthree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqfour$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eqfive$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.25,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eeu$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.25,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eev$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(-1.25,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eey$
%</text>
%<multicurve fill-style= "none"
%	 points= "(3.76,13.75);(3.76,13.75);(6.26,13.75);(6.26,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.76,11.25);(3.76,11.25);(6.26,11.25);(6.26,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.26,13.75);(6.26,13.75);(6.26,11.25);(6.26,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.76,13.75);(3.76,13.75);(3.76,11.25);(3.76,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.76,8.75);(8.76,8.75);(11.26,8.75);(11.26,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.76,6.25);(8.76,6.25);(11.26,6.25);(11.26,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.26,8.75);(11.26,8.75);(11.26,6.25);(11.26,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.76,8.75);(8.76,8.75);(8.76,6.25);(8.76,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(28.75,8.75);(28.75,8.75);(28.75,6.25);(28.75,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(31.25,6.25);(31.25,6.25);(35,2.5);(35,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(28.75,6.25);(28.75,6.25);(25,2.5);(25,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,11.25);(30,11.25);(30,8.75);(30,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(28.75,6.25);(28.75,6.25);(31.25,6.25);(31.25,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(28.75,8.75);(28.75,8.75);(31.25,8.75);(31.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(31.25,6.25);(31.25,6.25);(31.25,8.75);(31.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,17.5);(25,17.5);(28.75,13.75);(28.75,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,17.5);(35,17.5);(31.25,13.75);(31.25,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,20);(25,20);(25,17.5);(25,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,20);(35,20);(35,17.5);(35,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(96.25,15);(96.25,15);(98.75,12.5);(98.75,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,15);(93.75,15);(91.25,12.5);(91.25,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,2.5);(95,2.5);(95,0);(95,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(91.25,12.5);(91.25,12.5);(91.25,7.5);(91.25,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(98.75,12.5);(98.75,12.5);(98.75,7.5);(98.75,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(91.25,7.5);(91.25,7.5);(93.75,5);(93.75,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(98.75,7.5);(98.75,7.5);(96.25,5);(96.25,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,20);(110,20);(110,0);(110,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(105,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\SUB
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\SUB
%</text>
%<multicurve fill-style= "none"
%	 points= "(28.75,13.75);(28.75,13.75);(28.75,11.25);(28.75,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(28.75,11.25);(28.75,11.25);(31.25,11.25);(31.25,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(28.75,13.75);(28.75,13.75);(31.25,13.75);(31.25,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(31.25,11.25);(31.25,11.25);(31.25,13.75);(31.25,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,17.5);(93.75,17.5);(93.75,15);(93.75,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,15);(93.75,15);(96.25,15);(96.25,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,17.5);(93.75,17.5);(96.25,17.5);(96.25,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(96.25,15);(96.25,15);(96.25,17.5);(96.25,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,5);(93.75,5);(93.75,2.5);(93.75,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,2.5);(93.75,2.5);(96.25,2.5);(96.25,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,5);(93.75,5);(96.25,5);(96.25,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(96.25,2.5);(96.25,2.5);(96.25,5);(96.25,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,2.5);(25,2.5);(25,0);(25,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,2.5);(35,2.5);(35,0);(35,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\SUP
%</text>
%<multicurve fill-style= "none"
%	 points= "(45,20);(45,20);(45,12.5);(45,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,6.25);(50,6.25);(50,0);(50,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,7.5);(60,7.5);(60,0);(60,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,12.5);(45,12.5);(48.75,8.75);(48.75,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(51.25,8.75);(51.25,8.75);(53.75,11.25);(53.75,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(56.25,11.25);(56.25,11.25);(60,7.5);(60,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,20);(55,20);(54.99,13.75);(54.99,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(53.75,13.75);(53.75,13.75);(56.25,13.75);(56.25,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(53.75,11.25);(53.75,11.25);(56.25,11.25);(56.25,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(56.25,13.75);(56.25,13.75);(56.25,11.25);(56.25,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(53.75,13.75);(53.75,13.75);(53.75,11.25);(53.75,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(48.75,8.75);(48.75,8.75);(51.25,8.75);(51.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(48.75,6.25);(48.75,6.25);(51.25,6.25);(51.25,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(51.25,8.75);(51.25,8.75);(51.25,6.25);(51.25,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(48.75,8.75);(48.75,8.75);(48.75,6.25);(48.75,6.25)"
%	 />
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(8.12,10.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\ees$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(51.88,10.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eet$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(26.25,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eeu$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(36.25,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eev$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(46.25,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eeu$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(56.25,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eev$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(23.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(33.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eey$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(48.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(58.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eey$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\THEN
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\IF
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(105,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\THEN
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(31.25,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eew$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(90,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eeu$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eev$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(93.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(96.25,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eey$
%</text>
%<multicurve fill-style= "none"
%	 points= "(95,20);(95,20);(95,17.5);(95,17.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(108.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(111.25,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eey$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(111.25,30)
\rput(10,30){$\eqone$}
\rput(30,30){$\eqtwo$}
\psline(15,20)(15,12.5)
\psline(10,6.25)(10,0)
\psline(0.01,7.5)(0,0)
\psline(15,12.5)(11.25,8.75)
\psline(0.01,7.5)(3.76,11.25)
\psline(6.26,11.25)(8.76,8.75)
\psline(5,20)(4.99,13.75)
\rput(50,30){$\eqthree$}
\rput(95,30){$\eqfour$}
\rput[l](110,30){$\eqfive$}
\rput[l](6.25,20){$\eeu$}
\rput[l](16.25,20){$\eev$}
\rput[r](-1.25,0){$\eex$}
\rput[r](8.75,0){$\eey$}
\psline(3.76,13.75)(6.26,13.75)
\psline(3.76,11.25)(6.26,11.25)
\psline(6.26,13.75)(6.26,11.25)
\psline(3.76,13.75)(3.76,11.25)
\psline(8.76,8.75)(11.26,8.75)
\psline(8.76,6.25)(11.26,6.25)
\psline(11.26,8.75)(11.26,6.25)
\psline(8.76,8.75)(8.76,6.25)
\psline(28.75,8.75)(28.75,6.25)
\psline(31.25,6.25)(35,2.5)
\psline(28.75,6.25)(25,2.5)
\psline(30,11.25)(30,8.75)
\psline(28.75,6.25)(31.25,6.25)
\psline(28.75,8.75)(31.25,8.75)
\psline(31.25,6.25)(31.25,8.75)
\psline(25,17.5)(28.75,13.75)
\psline(35,17.5)(31.25,13.75)
\psline(25,20)(25,17.5)
\psline(35,20)(35,17.5)
\psline(96.25,15)(98.75,12.5)
\psline(93.75,15)(91.25,12.5)
\psline(95,2.5)(95,0)
\psline(91.25,12.5)(91.25,7.5)
\psline(98.75,12.5)(98.75,7.5)
\psline(91.25,7.5)(93.75,5)
\psline(98.75,7.5)(96.25,5)
\psline(110,20)(110,0)
\rput(105,10){\SUB}
\rput(40,10){\SUB}
\psline(28.75,13.75)(28.75,11.25)
\psline(28.75,11.25)(31.25,11.25)
\psline(28.75,13.75)(31.25,13.75)
\psline(31.25,11.25)(31.25,13.75)
\psline(93.75,17.5)(93.75,15)
\psline(93.75,15)(96.25,15)
\psline(93.75,17.5)(96.25,17.5)
\psline(96.25,15)(96.25,17.5)
\psline(93.75,5)(93.75,2.5)
\psline(93.75,2.5)(96.25,2.5)
\psline(93.75,5)(96.25,5)
\psline(96.25,2.5)(96.25,5)
\psline(25,2.5)(25,0)
\psline(35,2.5)(35,0)
\rput(20,10){\SUP}
\psline(45,20)(45,12.5)
\psline(50,6.25)(50,0)
\psline(60,7.5)(60,0)
\psline(45,12.5)(48.75,8.75)
\psline(51.25,8.75)(53.75,11.25)
\psline(56.25,11.25)(60,7.5)
\psline(55,20)(54.99,13.75)
\psline(53.75,13.75)(56.25,13.75)
\psline(53.75,11.25)(56.25,11.25)
\psline(56.25,13.75)(56.25,11.25)
\psline(53.75,13.75)(53.75,11.25)
\psline(48.75,8.75)(51.25,8.75)
\psline(48.75,6.25)(51.25,6.25)
\psline(51.25,8.75)(51.25,6.25)
\psline(48.75,8.75)(48.75,6.25)
\rput[bl](8.12,10.62){$\ees$}
\rput[br](51.88,10.62){$\eet$}
\rput[l](26.25,20){$\eeu$}
\rput[l](36.25,20){$\eev$}
\rput[l](46.25,20){$\eeu$}
\rput[l](56.25,20){$\eev$}
\rput[r](23.75,0){$\eex$}
\rput[r](33.75,0){$\eey$}
\rput[r](48.75,0){$\eex$}
\rput[r](58.75,0){$\eey$}
\rput(40,30){\THEN}
\rput(20,30){\IF}
\rput(105,30){\THEN}
\rput[l](31.25,10){$\eew$}
\rput[r](90,10){$\eeu$}
\rput[l](100,10){$\eev$}
\rput[r](93.75,0){$\eex$}
\rput[l](96.25,20){$\eey$}
\psline(95,20)(95,17.5)
\rput[r](108.75,0){$\eex$}
\rput[l](111.25,20){$\eey$}
\end{pspicture}


==> PIC/monoid-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Apr 20 18:57:51 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-1.87" x-max="121.25" y-min="0" y-max="27.5" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25.63,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eqone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(31.87,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eqtwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(28.75,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,5);(0,5);(0,0);(0,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,5);(10,5);(10,0);(10,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,10);(15,10);(15,0);(15,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,10);(5,10);(10,5);(10,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,5);(0,5);(10,15);(10,15)"
%	 />
%<ellipse p3= "(8.98,16.02)"
%	 fill-style= "none"
%	 p2= "(8.98,13.98)"
%	 p1= "(11.02,13.98)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,15);(10,15);(15,10);(15,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,20);(10,20);(10,15);(10,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60.63,5);(60.63,5);(60.63,0);(60.63,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50.63,5);(50.63,5);(50.63,0);(50.63,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45.63,10);(45.63,10);(45.63,0);(45.63,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55.63,10);(55.63,10);(50.63,5);(50.63,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45.63,10);(45.63,10);(50.63,15);(50.63,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50.63,15);(50.63,15);(60.63,5);(60.63,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50.63,20);(50.63,20);(50.63,15);(50.63,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(91.25,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(86.25,10);(86.25,10);(86.25,0);(86.25,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(76.25,10);(76.25,10);(81.25,15);(81.25,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(81.25,15);(81.25,15);(86.25,10);(86.25,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(81.25,20);(81.25,20);(81.25,15);(81.25,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,20);(120,20);(120,0);(120,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(96.25,10);(96.25,10);(96.25,0);(96.25,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(96.25,10);(96.25,10);(101.25,15);(101.25,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(101.25,15);(101.25,15);(106.25,10);(106.25,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(101.25,20);(101.25,20);(101.25,15);(101.25,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(111.25,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(88.13,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eqthree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(101.25,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqfour$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(114.37,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eqfive$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(91.25,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\IFF
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(28.75,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\IFF
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(111.25,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\IFF
%</text>
%<ellipse p3= "(80.23,16.02)"
%	 fill-style= "none"
%	 p2= "(80.23,13.98)"
%	 p1= "(82.27,13.98)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 right-arrow= "head"
%	 />
%<ellipse p3= "(75.23,11.02)"
%	 fill-style= "none"
%	 p2= "(75.23,8.98)"
%	 p1= "(77.27,8.98)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 right-arrow= "head"
%	 />
%<ellipse p3= "(105.23,11.02)"
%	 fill-style= "none"
%	 p2= "(105.23,8.98)"
%	 p1= "(107.27,8.98)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 right-arrow= "head"
%	 />
%<ellipse p3= "(100.23,16.02)"
%	 fill-style= "none"
%	 p2= "(100.23,13.98)"
%	 p1= "(102.27,13.98)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 right-arrow= "head"
%	 />
%<ellipse p3= "(49.61,16.02)"
%	 fill-style= "none"
%	 p2= "(49.61,13.98)"
%	 p1= "(51.64,13.98)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 right-arrow= "head"
%	 />
%<ellipse p3= "(54.61,11.02)"
%	 fill-style= "none"
%	 p2= "(54.61,8.98)"
%	 p1= "(56.64,8.98)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 right-arrow= "head"
%	 />
%<ellipse p3= "(3.98,11.02)"
%	 fill-style= "none"
%	 p2= "(3.98,8.98)"
%	 p1= "(6.02,8.98)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(-1.87,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eey$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eez$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(6.87,13.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eeu$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(53.75,13.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eev$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(51.87,19.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eew$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(11.25,19.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eew$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(44.37,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(85,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(118.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(49.37,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eey$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(82.5,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eey$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(102.5,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eey$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(121.25,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eey$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(59.37,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eez$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(121.25,27.5)
\rput[r](25.63,27.5){$\eqone$}
\rput[l](31.87,27.5){$\eqtwo$}
\rput(28.75,10){\EQLS}
\psline(0,5)(0,0)
\psline(10,5)(10,0)
\psline(15,10)(15,0)
\psline(5,10)(10,5)
\psline(0,5)(10,15)
\rput{0}(10,15){\psellipse[](0,0)(1.02,-1.02)}
\psline(10,15)(15,10)
\psline(10,20)(10,15)
\psline(60.63,5)(60.63,0)
\psline(50.63,5)(50.63,0)
\psline(45.63,10)(45.63,0)
\psline(55.63,10)(50.63,5)
\psline(45.63,10)(50.63,15)
\psline(50.63,15)(60.63,5)
\psline(50.63,20)(50.63,15)
\rput(91.25,10){\EQLS}
\psline(86.25,10)(86.25,0)
\psline(76.25,10)(81.25,15)
\psline(81.25,15)(86.25,10)
\psline(81.25,20)(81.25,15)
\psline(120,20)(120,0)
\psline(96.25,10)(96.25,0)
\psline(96.25,10)(101.25,15)
\psline(101.25,15)(106.25,10)
\psline(101.25,20)(101.25,15)
\rput(111.25,10){\EQLS}
\rput[r](88.13,27.5){$\eqthree$}
\rput(101.25,27.5){$\eqfour$}
\rput[l](114.37,27.5){$\eqfive$}
\rput(91.25,27.5){\IFF}
\rput(28.75,27.5){\IFF}
\rput(111.25,27.5){\IFF}
\rput{0}(81.25,15){\psellipse[](0,0)(1.02,-1.02)}
\rput{0}(76.25,10){\psellipse[](0,0)(1.02,-1.02)}
\rput{0}(106.25,10){\psellipse[](0,0)(1.02,-1.02)}
\rput{0}(101.25,15){\psellipse[](0,0)(1.02,-1.02)}
\rput{90}(50.62,15){\psellipse[](0,0)(1.02,-1.01)}
\rput{90}(55.62,10){\psellipse[](0,0)(1.02,-1.01)}
\rput{0}(5,10){\psellipse[](0,0)(1.02,-1.02)}
\rput[r](-1.87,0){$\eex$}
\rput[r](8.75,0){$\eey$}
\rput[r](13.75,0){$\eez$}
\rput[br](6.87,13.12){$\eeu$}
\rput[bl](53.75,13.12){$\eev$}
\rput[l](51.87,19.38){$\eew$}
\rput[l](11.25,19.38){$\eew$}
\rput[r](44.37,0){$\eex$}
\rput[r](85,0){$\eex$}
\rput[r](95,0){$\eex$}
\rput[r](118.75,0){$\eex$}
\rput[r](49.37,0){$\eey$}
\rput[l](82.5,20){$\eey$}
\rput[l](102.5,20){$\eey$}
\rput[l](121.25,20){$\eey$}
\rput[r](59.37,0){$\eez$}
\end{pspicture}


==> PIC/monoid-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Apr 20 19:01:48 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-1.87" x-max="121.25" y-min="0" y-max="27.5" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25.63,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eqone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(31.87,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eqtwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(28.75,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,5);(0,5);(0,0);(0,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,5);(10,5);(10,0);(10,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,10);(15,10);(15,0);(15,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5.62,9.38);(5.62,9.38);(10,5);(10,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5.62,10.62);(5.62,10.62);(9.38,14.38);(9.38,14.38)"
%	 />
%<ellipse p3= "(8.98,16.02)"
%	 fill-style= "none"
%	 p2= "(8.98,13.98)"
%	 p1= "(11.02,13.98)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10.62,14.38);(10.62,14.38);(15,10);(15,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,20);(10,20);(10,16.25);(10,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60.63,5);(60.63,5);(60.63,0);(60.63,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50.63,5);(50.63,5);(50.63,0);(50.63,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45.63,10);(45.63,10);(45.63,0);(45.63,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,9.38);(55,9.38);(50.63,5);(50.63,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45.63,10);(45.63,10);(50,14.38);(50,14.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(51.25,14.38);(51.25,14.38);(55,10.62);(55,10.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50.63,20);(50.63,20);(50.62,16.25);(50.62,16.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(91.25,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(86.25,10);(86.25,10);(86.25,0);(86.25,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(76.88,10.62);(76.88,10.62);(80.62,14.38);(80.62,14.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(81.88,14.38);(81.88,14.38);(86.25,10);(86.25,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(81.25,20);(81.25,20);(81.25,16.25);(81.25,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,20);(120,20);(120,0);(120,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(96.25,10);(96.25,10);(96.25,0);(96.25,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(96.25,10);(96.25,10);(100.62,14.38);(100.62,14.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(101.88,14.38);(101.88,14.38);(105.62,10.62);(105.62,10.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(101.25,20);(101.25,20);(101.25,16.25);(101.25,16.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(111.25,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(88.13,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eqthree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(101.25,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqfour$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(114.37,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eqfive$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(91.25,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\IFF
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(28.75,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\IFF
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(111.25,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\IFF
%</text>
%<ellipse p3= "(80.23,16.02)"
%	 fill-style= "none"
%	 p2= "(80.23,13.98)"
%	 p1= "(82.27,13.98)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 right-arrow= "head"
%	 />
%<ellipse p3= "(75.23,11.02)"
%	 fill-style= "none"
%	 p2= "(75.23,8.98)"
%	 p1= "(77.27,8.98)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 right-arrow= "head"
%	 />
%<ellipse p3= "(105.23,11.02)"
%	 fill-style= "none"
%	 p2= "(105.23,8.98)"
%	 p1= "(107.27,8.98)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 right-arrow= "head"
%	 />
%<ellipse p3= "(100.23,16.02)"
%	 fill-style= "none"
%	 p2= "(100.23,13.98)"
%	 p1= "(102.27,13.98)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 right-arrow= "head"
%	 />
%<ellipse p3= "(49.61,16.02)"
%	 fill-style= "none"
%	 p2= "(49.61,13.98)"
%	 p1= "(51.64,13.98)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 right-arrow= "head"
%	 />
%<ellipse p3= "(54.61,11.02)"
%	 fill-style= "none"
%	 p2= "(54.61,8.98)"
%	 p1= "(56.64,8.98)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 right-arrow= "head"
%	 />
%<ellipse p3= "(3.98,11.02)"
%	 fill-style= "none"
%	 p2= "(3.98,8.98)"
%	 p1= "(6.02,8.98)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(-1.87,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eey$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eez$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(6.87,13.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eeu$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(53.75,13.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eev$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(51.87,19.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eew$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(11.25,19.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eew$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(44.37,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(85,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(118.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(49.37,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eey$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(82.5,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eey$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(102.5,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eey$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(121.25,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eey$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(59.37,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eez$
%</text>
%<multicurve fill-style= "none"
%	 points= "(56.25,9.38);(56.25,9.38);(60.62,5);(60.62,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,5);(0,5);(4.38,9.38);(4.38,9.38)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(121.25,27.5)
\rput[r](25.63,27.5){$\eqone$}
\rput[l](31.87,27.5){$\eqtwo$}
\rput(28.75,10){\EQLS}
\psline(0,5)(0,0)
\psline(10,5)(10,0)
\psline(15,10)(15,0)
\psline(5.62,9.38)(10,5)
\psline(5.62,10.62)(9.38,14.38)
\rput{0}(10,15){\psellipse[](0,0)(1.02,-1.02)}
\psline(10.62,14.38)(15,10)
\psline(10,20)(10,16.25)
\psline(60.63,5)(60.63,0)
\psline(50.63,5)(50.63,0)
\psline(45.63,10)(45.63,0)
\psline(55,9.38)(50.63,5)
\psline(45.63,10)(50,14.38)
\psline(51.25,14.38)(55,10.62)
\psline(50.63,20)(50.62,16.25)
\rput(91.25,10){\EQLS}
\psline(86.25,10)(86.25,0)
\psline(76.88,10.62)(80.62,14.38)
\psline(81.88,14.38)(86.25,10)
\psline(81.25,20)(81.25,16.25)
\psline(120,20)(120,0)
\psline(96.25,10)(96.25,0)
\psline(96.25,10)(100.62,14.38)
\psline(101.88,14.38)(105.62,10.62)
\psline(101.25,20)(101.25,16.25)
\rput(111.25,10){\EQLS}
\rput[r](88.13,27.5){$\eqthree$}
\rput(101.25,27.5){$\eqfour$}
\rput[l](114.37,27.5){$\eqfive$}
\rput(91.25,27.5){\IFF}
\rput(28.75,27.5){\IFF}
\rput(111.25,27.5){\IFF}
\rput{0}(81.25,15){\psellipse[](0,0)(1.02,-1.02)}
\rput{0}(76.25,10){\psellipse[](0,0)(1.02,-1.02)}
\rput{0}(106.25,10){\psellipse[](0,0)(1.02,-1.02)}
\rput{0}(101.25,15){\psellipse[](0,0)(1.02,-1.02)}
\rput{90}(50.62,15){\psellipse[](0,0)(1.02,-1.01)}
\rput{90}(55.62,10){\psellipse[](0,0)(1.02,-1.01)}
\rput{0}(5,10){\psellipse[](0,0)(1.02,-1.02)}
\rput[r](-1.87,0){$\eex$}
\rput[r](8.75,0){$\eey$}
\rput[r](13.75,0){$\eez$}
\rput[br](6.87,13.12){$\eeu$}
\rput[bl](53.75,13.12){$\eev$}
\rput[l](51.87,19.38){$\eew$}
\rput[l](11.25,19.38){$\eew$}
\rput[r](44.37,0){$\eex$}
\rput[r](85,0){$\eex$}
\rput[r](95,0){$\eex$}
\rput[r](118.75,0){$\eex$}
\rput[r](49.37,0){$\eey$}
\rput[l](82.5,20){$\eey$}
\rput[l](102.5,20){$\eey$}
\rput[l](121.25,20){$\eey$}
\rput[r](59.37,0){$\eez$}
\psline(56.25,9.38)(60.62,5)
\psline(0,5)(4.38,9.38)
\end{pspicture}


==> PIC/monoid.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Apr 20 21:21:28 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-1.87" x-max="121.25" y-min="0" y-max="27.5" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25.63,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eqone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(31.87,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eqtwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(28.75,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,5);(0,5);(0,0);(0,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,5);(10,5);(10,0);(10,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,10);(15,10);(15,0);(15,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.25,8.75);(6.25,8.75);(10,5);(10,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.25,11.25);(6.25,11.25);(8.75,13.75);(8.75,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,13.75);(11.25,13.75);(15,10);(15,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,20);(10,20);(10,16.25);(10,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60.63,5);(60.63,5);(60.63,0);(60.63,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50.63,5);(50.63,5);(50.63,0);(50.63,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45.63,10);(45.63,10);(45.63,0);(45.63,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(54.38,8.75);(54.38,8.75);(50.63,5);(50.63,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45.63,10);(45.63,10);(49.38,13.75);(49.38,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(51.88,13.75);(51.88,13.75);(54.38,11.25);(54.38,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50.63,20);(50.63,20);(50.62,16.25);(50.62,16.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(91.25,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(86.25,10);(86.25,10);(86.25,0);(86.25,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(77.5,11.25);(77.5,11.25);(80,13.75);(80,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(82.5,13.75);(82.5,13.75);(86.25,10);(86.25,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(81.25,20);(81.25,20);(81.25,16.25);(81.25,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,20);(120,20);(120,0);(120,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(96.25,10);(96.25,10);(96.25,0);(96.25,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(96.25,10);(96.25,10);(100,13.75);(100,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,13.75);(102.5,13.75);(105,11.25);(105,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(101.25,20);(101.25,20);(101.25,16.25);(101.25,16.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(111.25,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(88.13,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eqthree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(101.25,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqfour$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(114.37,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eqfive$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(91.25,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\IFF
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(28.75,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\IFF
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(111.25,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\IFF
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(-1.87,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eey$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eez$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(6.87,13.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eeu$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(53.75,13.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eev$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(51.87,19.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eew$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(11.25,19.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eew$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(44.37,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(85,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(118.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(49.37,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eey$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(82.5,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eey$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(102.5,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eey$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(121.25,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eey$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(59.37,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eez$
%</text>
%<multicurve fill-style= "none"
%	 points= "(56.88,8.75);(56.88,8.75);(60.62,5);(60.62,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,5);(0,5);(3.75,8.75);(3.75,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.75,16.25);(8.75,16.25);(11.25,16.25);(11.25,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.75,13.75);(8.75,13.75);(11.25,13.75);(11.25,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,16.25);(11.25,16.25);(11.25,13.75);(11.25,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.75,16.25);(8.75,16.25);(8.75,13.75);(8.75,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(49.38,16.25);(49.38,16.25);(51.88,16.25);(51.88,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(49.38,13.75);(49.38,13.75);(51.88,13.75);(51.88,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(51.88,16.25);(51.88,16.25);(51.88,13.75);(51.88,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(49.38,16.25);(49.38,16.25);(49.38,13.75);(49.38,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,11.25);(3.75,11.25);(6.25,11.25);(6.25,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,8.75);(3.75,8.75);(6.25,8.75);(6.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.25,11.25);(6.25,11.25);(6.25,8.75);(6.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,11.25);(3.75,11.25);(3.75,8.75);(3.75,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(54.38,11.25);(54.38,11.25);(56.88,11.25);(56.88,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(54.38,8.75);(54.38,8.75);(56.88,8.75);(56.88,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(56.88,11.25);(56.88,11.25);(56.88,8.75);(56.88,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(54.38,11.25);(54.38,11.25);(54.38,8.75);(54.38,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,11.25);(75,11.25);(77.5,11.25);(77.5,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,8.75);(75,8.75);(77.5,8.75);(77.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(77.5,11.25);(77.5,11.25);(77.5,8.75);(77.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,11.25);(75,11.25);(75,8.75);(75,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,16.25);(80,16.25);(82.5,16.25);(82.5,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,13.75);(80,13.75);(82.5,13.75);(82.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(82.5,16.25);(82.5,16.25);(82.5,13.75);(82.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,16.25);(80,16.25);(80,13.75);(80,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,16.25);(100,16.25);(102.5,16.25);(102.5,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,13.75);(100,13.75);(102.5,13.75);(102.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,16.25);(102.5,16.25);(102.5,13.75);(102.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,16.25);(100,16.25);(100,13.75);(100,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,11.25);(105,11.25);(107.5,11.25);(107.5,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,8.75);(105,8.75);(107.5,8.75);(107.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,11.25);(107.5,11.25);(107.5,8.75);(107.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,11.25);(105,11.25);(105,8.75);(105,8.75)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(121.25,27.5)
\rput[r](25.63,27.5){$\eqone$}
\rput[l](31.87,27.5){$\eqtwo$}
\rput(28.75,10){\EQLS}
\psline(0,5)(0,0)
\psline(10,5)(10,0)
\psline(15,10)(15,0)
\psline(6.25,8.75)(10,5)
\psline(6.25,11.25)(8.75,13.75)
\psline(11.25,13.75)(15,10)
\psline(10,20)(10,16.25)
\psline(60.63,5)(60.63,0)
\psline(50.63,5)(50.63,0)
\psline(45.63,10)(45.63,0)
\psline(54.38,8.75)(50.63,5)
\psline(45.63,10)(49.38,13.75)
\psline(51.88,13.75)(54.38,11.25)
\psline(50.63,20)(50.62,16.25)
\rput(91.25,10){\EQLS}
\psline(86.25,10)(86.25,0)
\psline(77.5,11.25)(80,13.75)
\psline(82.5,13.75)(86.25,10)
\psline(81.25,20)(81.25,16.25)
\psline(120,20)(120,0)
\psline(96.25,10)(96.25,0)
\psline(96.25,10)(100,13.75)
\psline(102.5,13.75)(105,11.25)
\psline(101.25,20)(101.25,16.25)
\rput(111.25,10){\EQLS}
\rput[r](88.13,27.5){$\eqthree$}
\rput(101.25,27.5){$\eqfour$}
\rput[l](114.37,27.5){$\eqfive$}
\rput(91.25,27.5){\IFF}
\rput(28.75,27.5){\IFF}
\rput(111.25,27.5){\IFF}
\rput[r](-1.87,0){$\eex$}
\rput[r](8.75,0){$\eey$}
\rput[r](13.75,0){$\eez$}
\rput[br](6.87,13.12){$\eeu$}
\rput[bl](53.75,13.12){$\eev$}
\rput[l](51.87,19.38){$\eew$}
\rput[l](11.25,19.38){$\eew$}
\rput[r](44.37,0){$\eex$}
\rput[r](85,0){$\eex$}
\rput[r](95,0){$\eex$}
\rput[r](118.75,0){$\eex$}
\rput[r](49.37,0){$\eey$}
\rput[l](82.5,20){$\eey$}
\rput[l](102.5,20){$\eey$}
\rput[l](121.25,20){$\eey$}
\rput[r](59.37,0){$\eez$}
\psline(56.88,8.75)(60.62,5)
\psline(0,5)(3.75,8.75)
\psline(8.75,16.25)(11.25,16.25)
\psline(8.75,13.75)(11.25,13.75)
\psline(11.25,16.25)(11.25,13.75)
\psline(8.75,16.25)(8.75,13.75)
\psline(49.38,16.25)(51.88,16.25)
\psline(49.38,13.75)(51.88,13.75)
\psline(51.88,16.25)(51.88,13.75)
\psline(49.38,16.25)(49.38,13.75)
\psline(3.75,11.25)(6.25,11.25)
\psline(3.75,8.75)(6.25,8.75)
\psline(6.25,11.25)(6.25,8.75)
\psline(3.75,11.25)(3.75,8.75)
\psline(54.38,11.25)(56.88,11.25)
\psline(54.38,8.75)(56.88,8.75)
\psline(56.88,11.25)(56.88,8.75)
\psline(54.38,11.25)(54.38,8.75)
\psline(75,11.25)(77.5,11.25)
\psline(75,8.75)(77.5,8.75)
\psline(77.5,11.25)(77.5,8.75)
\psline(75,11.25)(75,8.75)
\psline(80,16.25)(82.5,16.25)
\psline(80,13.75)(82.5,13.75)
\psline(82.5,16.25)(82.5,13.75)
\psline(80,16.25)(80,13.75)
\psline(100,16.25)(102.5,16.25)
\psline(100,13.75)(102.5,13.75)
\psline(102.5,16.25)(102.5,13.75)
\psline(100,16.25)(100,13.75)
\psline(105,11.25)(107.5,11.25)
\psline(105,8.75)(107.5,8.75)
\psline(107.5,11.25)(107.5,8.75)
\psline(105,11.25)(105,8.75)
\end{pspicture}


==> PIC/preg-map-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Apr 20 21:15:42 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.25" x-max="120" y-min="0" y-max="27.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(33.75,11.25);(33.75,11.25);(33.75,8.75);(33.75,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(36.25,8.75);(36.25,8.75);(40,5);(40,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,8.75);(33.75,8.75);(30,5);(30,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.25,27.5);(1.25,27.5);(1.25,0);(1.25,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,16.25);(35,16.25);(35,11.25);(35,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,8.75);(33.75,8.75);(36.25,8.75);(36.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,11.25);(33.75,11.25);(36.25,11.25);(36.25,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(36.25,8.75);(36.25,8.75);(36.25,11.25);(36.25,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.75,27.5);(8.75,27.5);(8.75,0);(8.75,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,5);(30,5);(30,0);(30,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,5);(40,5);(40,0);(40,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,22.5);(30,22.5);(33.75,18.75);(33.75,18.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,22.5);(40,22.5);(36.25,18.75);(36.25,18.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,27.5);(30,27.5);(30,22.5);(30,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,27.5);(40,27.5);(40,22.5);(40,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(96.25,21.25);(96.25,21.25);(100,17.5);(100,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,21.25);(93.75,21.25);(90,17.5);(90,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,3.75);(95,3.75);(95,0);(95,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,17.5);(90,17.5);(90,10);(90,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,17.5);(100,17.5);(100,10);(100,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,10);(90,10);(93.75,6.25);(93.75,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,10);(100,10);(96.25,6.25);(96.25,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,27.5);(95,27.5);(95,23.75);(95,23.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,27.5);(120,27.5);(120,0);(120,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\SUB
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\SUB
%</text>
%<multicurve fill-style= "none"
%	 points= "(33.75,18.75);(33.75,18.75);(33.75,16.25);(33.75,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,16.25);(33.75,16.25);(36.25,16.25);(36.25,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,18.75);(33.75,18.75);(36.25,18.75);(36.25,18.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(36.25,16.25);(36.25,16.25);(36.25,18.75);(36.25,18.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,23.75);(93.75,23.75);(93.75,21.25);(93.75,21.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,21.25);(93.75,21.25);(96.25,21.25);(96.25,21.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,23.75);(93.75,23.75);(96.25,23.75);(96.25,23.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(96.25,21.25);(96.25,21.25);(96.25,23.75);(96.25,23.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,6.25);(93.75,6.25);(93.75,3.75);(93.75,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,3.75);(93.75,3.75);(96.25,3.75);(96.25,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,6.25);(93.75,6.25);(96.25,6.25);(96.25,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(96.25,3.75);(96.25,3.75);(96.25,6.25);(96.25,6.25)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(120,27.5)
\psline(33.75,11.25)(33.75,8.75)
\psline(36.25,8.75)(40,5)
\psline(33.75,8.75)(30,5)
\psline(1.25,27.5)(1.25,0)
\psline(35,16.25)(35,11.25)
\psline(33.75,8.75)(36.25,8.75)
\psline(33.75,11.25)(36.25,11.25)
\psline(36.25,8.75)(36.25,11.25)
\psline(8.75,27.5)(8.75,0)
\psline(30,5)(30,0)
\psline(40,5)(40,0)
\psline(30,22.5)(33.75,18.75)
\psline(40,22.5)(36.25,18.75)
\psline(30,27.5)(30,22.5)
\psline(40,27.5)(40,22.5)
\psline(96.25,21.25)(100,17.5)
\psline(93.75,21.25)(90,17.5)
\psline(95,3.75)(95,0)
\psline(90,17.5)(90,10)
\psline(100,17.5)(100,10)
\psline(90,10)(93.75,6.25)
\psline(100,10)(96.25,6.25)
\psline(95,27.5)(95,23.75)
\psline(120,27.5)(120,0)
\rput(110,13.75){\SUB}
\rput(20,13.75){\SUB}
\psline(33.75,18.75)(33.75,16.25)
\psline(33.75,16.25)(36.25,16.25)
\psline(33.75,18.75)(36.25,18.75)
\psline(36.25,16.25)(36.25,18.75)
\psline(93.75,23.75)(93.75,21.25)
\psline(93.75,21.25)(96.25,21.25)
\psline(93.75,23.75)(96.25,23.75)
\psline(96.25,21.25)(96.25,23.75)
\psline(93.75,6.25)(93.75,3.75)
\psline(93.75,3.75)(96.25,3.75)
\psline(93.75,6.25)(96.25,6.25)
\psline(96.25,3.75)(96.25,6.25)
\end{pspicture}


==> PIC/preg-map-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Apr 20 21:21:24 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.25" x-max="120" y-min="0" y-max="27.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(33.75,11.25);(33.75,11.25);(33.75,8.75);(33.75,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(36.25,8.75);(36.25,8.75);(40,5);(40,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,8.75);(33.75,8.75);(30,5);(30,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.25,27.5);(1.25,27.5);(1.25,0);(1.25,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,16.25);(35,16.25);(35,11.25);(35,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,8.75);(33.75,8.75);(36.25,8.75);(36.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,11.25);(33.75,11.25);(36.25,11.25);(36.25,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(36.25,8.75);(36.25,8.75);(36.25,11.25);(36.25,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.75,27.5);(8.75,27.5);(8.75,0);(8.75,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,5);(30,5);(30,0);(30,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,5);(40,5);(40,0);(40,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,22.5);(30,22.5);(33.75,18.75);(33.75,18.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,22.5);(40,22.5);(36.25,18.75);(36.25,18.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,27.5);(30,27.5);(30,22.5);(30,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,27.5);(40,27.5);(40,22.5);(40,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(96.25,21.25);(96.25,21.25);(100,17.5);(100,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,21.25);(93.75,21.25);(90,17.5);(90,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,3.75);(95,3.75);(95,0);(95,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,17.5);(90,17.5);(90,10);(90,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,17.5);(100,17.5);(100,10);(100,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,10);(90,10);(93.75,6.25);(93.75,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,10);(100,10);(96.25,6.25);(96.25,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,27.5);(95,27.5);(95,23.75);(95,23.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,27.5);(120,27.5);(120,0);(120,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\SUB
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\SUB
%</text>
%<multicurve fill-style= "none"
%	 points= "(33.75,18.75);(33.75,18.75);(33.75,16.25);(33.75,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,16.25);(33.75,16.25);(36.25,16.25);(36.25,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,18.75);(33.75,18.75);(36.25,18.75);(36.25,18.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(36.25,16.25);(36.25,16.25);(36.25,18.75);(36.25,18.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,23.75);(93.75,23.75);(93.75,21.25);(93.75,21.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,21.25);(93.75,21.25);(96.25,21.25);(96.25,21.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,23.75);(93.75,23.75);(96.25,23.75);(96.25,23.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(96.25,21.25);(96.25,21.25);(96.25,23.75);(96.25,23.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,6.25);(93.75,6.25);(93.75,3.75);(93.75,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,3.75);(93.75,3.75);(96.25,3.75);(96.25,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,6.25);(93.75,6.25);(96.25,6.25);(96.25,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(96.25,3.75);(96.25,3.75);(96.25,6.25);(96.25,6.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pregr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\copregr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\copregr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pregr$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(120,27.5)
\psline(33.75,11.25)(33.75,8.75)
\psline(36.25,8.75)(40,5)
\psline(33.75,8.75)(30,5)
\psline(1.25,27.5)(1.25,0)
\psline(35,16.25)(35,11.25)
\psline(33.75,8.75)(36.25,8.75)
\psline(33.75,11.25)(36.25,11.25)
\psline(36.25,8.75)(36.25,11.25)
\psline(8.75,27.5)(8.75,0)
\psline(30,5)(30,0)
\psline(40,5)(40,0)
\psline(30,22.5)(33.75,18.75)
\psline(40,22.5)(36.25,18.75)
\psline(30,27.5)(30,22.5)
\psline(40,27.5)(40,22.5)
\psline(96.25,21.25)(100,17.5)
\psline(93.75,21.25)(90,17.5)
\psline(95,3.75)(95,0)
\psline(90,17.5)(90,10)
\psline(100,17.5)(100,10)
\psline(90,10)(93.75,6.25)
\psline(100,10)(96.25,6.25)
\psline(95,27.5)(95,23.75)
\psline(120,27.5)(120,0)
\rput(110,13.75){\SUB}
\rput(20,13.75){\SUB}
\psline(33.75,18.75)(33.75,16.25)
\psline(33.75,16.25)(36.25,16.25)
\psline(33.75,18.75)(36.25,18.75)
\psline(36.25,16.25)(36.25,18.75)
\psline(93.75,23.75)(93.75,21.25)
\psline(93.75,21.25)(96.25,21.25)
\psline(93.75,23.75)(96.25,23.75)
\psline(96.25,21.25)(96.25,23.75)
\psline(93.75,6.25)(93.75,3.75)
\psline(93.75,3.75)(96.25,3.75)
\psline(93.75,6.25)(96.25,6.25)
\psline(96.25,3.75)(96.25,6.25)
\rput(35,10){$\pregr$}
\rput(35,17.5){$\copregr$}
\rput(95,5){$\copregr$}
\rput(95,22.5){$\pregr$}
\end{pspicture}


==> PIC/preg-map.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Apr 20 21:08:14 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.25" x-max="120" y-min="0" y-max="40" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(33.75,13.75);(33.75,13.75);(33.75,11.25);(33.75,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(36.25,11.25);(36.25,11.25);(40,7.5);(40,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,11.25);(33.75,11.25);(30,7.5);(30,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.25,40);(1.25,40);(1.25,0);(1.25,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,26.25);(35,26.25);(35,13.75);(35,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,11.25);(33.75,11.25);(36.25,11.25);(36.25,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,13.75);(33.75,13.75);(36.25,13.75);(36.25,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(36.25,11.25);(36.25,11.25);(36.25,13.75);(36.25,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.75,40);(8.75,40);(8.75,0);(8.75,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,7.5);(30,7.5);(30,0);(30,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,7.5);(40,7.5);(40,0);(40,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,32.5);(30,32.5);(33.75,28.75);(33.75,28.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,32.5);(40,32.5);(36.25,28.75);(36.25,28.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,40);(30,40);(30,32.5);(30,32.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,40);(40,40);(40,32.5);(40,32.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(96.25,31.25);(96.25,31.25);(100,27.5);(100,27.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,31.25);(93.75,31.25);(90,27.5);(90,27.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,6.25);(95,6.25);(95,0);(95,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,27.5);(90,27.5);(90,12.5);(90,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,27.5);(100,27.5);(100,12.5);(100,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,12.5);(90,12.5);(93.75,8.75);(93.75,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,12.5);(100,12.5);(96.25,8.75);(96.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,40);(95,40);(95,33.75);(95,33.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,40);(120,40);(120,0);(120,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\SUB
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\SUB
%</text>
%<multicurve fill-style= "none"
%	 points= "(33.75,28.75);(33.75,28.75);(33.75,26.25);(33.75,26.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,26.25);(33.75,26.25);(36.25,26.25);(36.25,26.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,28.75);(33.75,28.75);(36.25,28.75);(36.25,28.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(36.25,26.25);(36.25,26.25);(36.25,28.75);(36.25,28.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,33.75);(93.75,33.75);(93.75,31.25);(93.75,31.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,31.25);(93.75,31.25);(96.25,31.25);(96.25,31.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,33.75);(93.75,33.75);(96.25,33.75);(96.25,33.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(96.25,31.25);(96.25,31.25);(96.25,33.75);(96.25,33.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,8.75);(93.75,8.75);(93.75,6.25);(93.75,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,6.25);(93.75,6.25);(96.25,6.25);(96.25,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,8.75);(93.75,8.75);(96.25,8.75);(96.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(96.25,6.25);(96.25,6.25);(96.25,8.75);(96.25,8.75)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(120,40)
\psline(33.75,13.75)(33.75,11.25)
\psline(36.25,11.25)(40,7.5)
\psline(33.75,11.25)(30,7.5)
\psline(1.25,40)(1.25,0)
\psline(35,26.25)(35,13.75)
\psline(33.75,11.25)(36.25,11.25)
\psline(33.75,13.75)(36.25,13.75)
\psline(36.25,11.25)(36.25,13.75)
\psline(8.75,40)(8.75,0)
\psline(30,7.5)(30,0)
\psline(40,7.5)(40,0)
\psline(30,32.5)(33.75,28.75)
\psline(40,32.5)(36.25,28.75)
\psline(30,40)(30,32.5)
\psline(40,40)(40,32.5)
\psline(96.25,31.25)(100,27.5)
\psline(93.75,31.25)(90,27.5)
\psline(95,6.25)(95,0)
\psline(90,27.5)(90,12.5)
\psline(100,27.5)(100,12.5)
\psline(90,12.5)(93.75,8.75)
\psline(100,12.5)(96.25,8.75)
\psline(95,40)(95,33.75)
\psline(120,40)(120,0)
\rput(110,20){\SUB}
\rput(20,20){\SUB}
\psline(33.75,28.75)(33.75,26.25)
\psline(33.75,26.25)(36.25,26.25)
\psline(33.75,28.75)(36.25,28.75)
\psline(36.25,26.25)(36.25,28.75)
\psline(93.75,33.75)(93.75,31.25)
\psline(93.75,31.25)(96.25,31.25)
\psline(93.75,33.75)(96.25,33.75)
\psline(96.25,31.25)(96.25,33.75)
\psline(93.75,8.75)(93.75,6.25)
\psline(93.75,6.25)(96.25,6.25)
\psline(93.75,8.75)(96.25,8.75)
\psline(96.25,6.25)(96.25,8.75)
\end{pspicture}


==> PIC/residues-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Apr 29 13:53:40 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-1.25" x-max="51.25" y-min="0" y-max="25" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(10,7.5);(10,7.5);(10,0);(10,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0.01,7.5);(0.01,7.5);(0,2.5);(0,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0.01,7.5);(0.01,7.5);(3.76,11.25);(3.76,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.26,11.25);(6.26,11.25);(10,7.5);(10,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,17.5);(5,17.5);(4.99,13.75);(4.99,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.76,13.75);(3.76,13.75);(6.26,13.75);(6.26,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.76,11.25);(3.76,11.25);(6.26,11.25);(6.26,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.26,13.75);(6.26,13.75);(6.26,11.25);(6.26,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.76,13.75);(3.76,13.75);(3.76,11.25);(3.76,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.25,2.5);(1.25,2.5);(1.25,0);(1.25,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-1.25,2.5);(-1.25,2.5);(-1.25,0);(-1.25,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-1.25,2.5);(-1.25,2.5);(1.25,2.5);(1.25,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-1.25,0);(-1.25,0);(1.25,0);(1.25,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(0,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\lugt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(6.25,20);(6.25,20);(6.25,17.5);(6.25,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,17.5);(3.75,17.5);(6.25,17.5);(6.25,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,20);(3.75,20);(6.25,20);(6.25,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,18.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prunt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(3.75,20);(3.75,20);(3.75,17.5);(3.75,17.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pregr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xil$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xir$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\rugt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,7.5);(40,7.5);(40,0);(40,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50.01,7.5);(50.01,7.5);(50,2.5);(50,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40.01,7.5);(40.01,7.5);(43.76,11.25);(43.76,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(46.26,11.25);(46.26,11.25);(50,7.5);(50,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,17.5);(45,17.5);(44.99,13.75);(44.99,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(43.76,13.75);(43.76,13.75);(46.26,13.75);(46.26,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(43.76,11.25);(43.76,11.25);(46.26,11.25);(46.26,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(46.26,13.75);(46.26,13.75);(46.26,11.25);(46.26,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(43.76,13.75);(43.76,13.75);(43.76,11.25);(43.76,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(51.25,2.5);(51.25,2.5);(51.25,0);(51.25,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(48.75,2.5);(48.75,2.5);(48.75,0);(48.75,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(48.75,2.5);(48.75,2.5);(51.25,2.5);(51.25,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(48.75,0);(48.75,0);(51.25,0);(51.25,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(46.25,20);(46.25,20);(46.25,17.5);(46.25,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(43.75,17.5);(43.75,17.5);(46.25,17.5);(46.25,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(43.75,20);(43.75,20);(46.25,20);(46.25,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45,18.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prunt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(43.75,20);(43.75,20);(43.75,17.5);(43.75,17.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pregr$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(51.25,25)
\psline(10,7.5)(10,0)
\psline(0.01,7.5)(0,2.5)
\psline(0.01,7.5)(3.76,11.25)
\psline(6.26,11.25)(10,7.5)
\psline(5,17.5)(4.99,13.75)
\psline(3.76,13.75)(6.26,13.75)
\psline(3.76,11.25)(6.26,11.25)
\psline(6.26,13.75)(6.26,11.25)
\psline(3.76,13.75)(3.76,11.25)
\psline(1.25,2.5)(1.25,0)
\psline(-1.25,2.5)(-1.25,0)
\psline(-1.25,2.5)(1.25,2.5)
\psline(-1.25,0)(1.25,0)
\rput(0,1.25){$\lugt$}
\psline(6.25,20)(6.25,17.5)
\psline(3.75,17.5)(6.25,17.5)
\psline(3.75,20)(6.25,20)
\rput(5,18.75){$\prunt$}
\psline(3.75,20)(3.75,17.5)
\rput(5,12.5){$\pregr$}
\rput(5,25){$\xil$}
\rput(45,25){$\xir$}
\rput(50,1.25){$\rugt$}
\psline(40,7.5)(40,0)
\psline(50.01,7.5)(50,2.5)
\psline(40.01,7.5)(43.76,11.25)
\psline(46.26,11.25)(50,7.5)
\psline(45,17.5)(44.99,13.75)
\psline(43.76,13.75)(46.26,13.75)
\psline(43.76,11.25)(46.26,11.25)
\psline(46.26,13.75)(46.26,11.25)
\psline(43.76,13.75)(43.76,11.25)
\psline(51.25,2.5)(51.25,0)
\psline(48.75,2.5)(48.75,0)
\psline(48.75,2.5)(51.25,2.5)
\psline(48.75,0)(51.25,0)
\psline(46.25,20)(46.25,17.5)
\psline(43.75,17.5)(46.25,17.5)
\psline(43.75,20)(46.25,20)
\rput(45,18.75){$\prunt$}
\psline(43.75,20)(43.75,17.5)
\rput(45,12.5){$\pregr$}
\end{pspicture}


==> PIC/residues-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Apr 30 08:51:38 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="35" y-min="0" y-max="17.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(35,17.5);(35,17.5);(35,12.5);(35,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,6.25);(30,6.25);(30,2.5);(30,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20.01,7.5);(20.01,7.5);(20,0);(20,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,12.5);(35,12.5);(31.25,8.75);(31.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20.01,7.5);(20.01,7.5);(23.76,11.25);(23.76,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(26.26,11.25);(26.26,11.25);(28.76,8.75);(28.76,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,17.5);(25,17.5);(24.99,13.75);(24.99,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(23.76,13.75);(23.76,13.75);(26.26,13.75);(26.26,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(23.76,11.25);(23.76,11.25);(26.26,11.25);(26.26,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(26.26,13.75);(26.26,13.75);(26.26,11.25);(26.26,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(23.76,13.75);(23.76,13.75);(23.76,11.25);(23.76,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(28.76,8.75);(28.76,8.75);(31.26,8.75);(31.26,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(28.76,6.25);(28.76,6.25);(31.26,6.25);(31.26,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(31.26,8.75);(31.26,8.75);(31.26,6.25);(31.26,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(28.76,8.75);(28.76,8.75);(28.76,6.25);(28.76,6.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fmnd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fcmn$
%</text>
%<multicurve fill-style= "none"
%	 points= "(31.25,2.5);(31.25,2.5);(31.25,0);(31.25,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(28.75,0);(28.75,0);(31.25,0);(31.25,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(28.75,2.5);(28.75,2.5);(31.25,2.5);(31.25,2.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prunt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(28.75,2.5);(28.75,2.5);(28.75,0);(28.75,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,8.75);(3.75,8.75);(3.75,6.25);(3.75,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,12.5);(0,12.5);(3.75,8.75);(3.75,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,12.5);(10,12.5);(6.25,8.75);(6.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,6.25);(5,6.25);(5,0);(5,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,6.25);(3.75,6.25);(6.25,6.25);(6.25,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,8.75);(3.75,8.75);(6.25,8.75);(6.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.25,6.25);(6.25,6.25);(6.25,8.75);(6.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,17.5);(10,17.5);(10,12.5);(10,12.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,8.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,17.5);(0,17.5);(0,12.5);(0,12.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fcmn$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(35,17.5)
\psline(35,17.5)(35,12.5)
\psline(30,6.25)(30,2.5)
\psline(20.01,7.5)(20,0)
\psline(35,12.5)(31.25,8.75)
\psline(20.01,7.5)(23.76,11.25)
\psline(26.26,11.25)(28.76,8.75)
\psline(25,17.5)(24.99,13.75)
\psline(23.76,13.75)(26.26,13.75)
\psline(23.76,11.25)(26.26,11.25)
\psline(26.26,13.75)(26.26,11.25)
\psline(23.76,13.75)(23.76,11.25)
\psline(28.76,8.75)(31.26,8.75)
\psline(28.76,6.25)(31.26,6.25)
\psline(31.26,8.75)(31.26,6.25)
\psline(28.76,8.75)(28.76,6.25)
\rput(25,12.5){$\fmnd$}
\rput(30,7.5){$\fcmn$}
\psline(31.25,2.5)(31.25,0)
\psline(28.75,0)(31.25,0)
\psline(28.75,2.5)(31.25,2.5)
\rput(30,1.25){$\prunt$}
\psline(28.75,2.5)(28.75,0)
\psline(3.75,8.75)(3.75,6.25)
\psline(0,12.5)(3.75,8.75)
\psline(10,12.5)(6.25,8.75)
\psline(5,6.25)(5,0)
\psline(3.75,6.25)(6.25,6.25)
\psline(3.75,8.75)(6.25,8.75)
\psline(6.25,6.25)(6.25,8.75)
\psline(10,17.5)(10,12.5)
\rput(15,8.75){\EQLS}
\psline(0,17.5)(0,12.5)
\rput(5,7.5){$\fcmn$}
\end{pspicture}


==> PIC/residues-frob.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Apr 29 13:48:07 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="3.75" x-max="55" y-min="0" y-max="25" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(11.25,15);(11.25,15);(11.25,12.5);(11.25,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.75,12.5);(8.75,12.5);(11.25,12.5);(11.25,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.75,15);(8.75,15);(11.25,15);(11.25,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prunt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(8.75,15);(8.75,15);(8.75,12.5);(8.75,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,8.75);(11.25,8.75);(15,5);(15,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.75,8.75);(8.75,8.75);(5,5);(5,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,2.5);(16.25,2.5);(16.25,0);(16.25,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,12.5);(10,12.5);(10,11.25);(10,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.75,11.25);(8.75,11.25);(8.75,8.75);(8.75,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.75,8.75);(8.75,8.75);(11.25,8.75);(11.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.75,11.25);(8.75,11.25);(11.25,11.25);(11.25,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,8.75);(11.25,8.75);(11.25,11.25);(11.25,11.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pregr$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,5);(5,5);(5,2.5);(5,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.25,2.5);(6.25,2.5);(6.25,0);(6.25,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,2.5);(3.75,2.5);(3.75,0);(3.75,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,2.5);(3.75,2.5);(6.25,2.5);(6.25,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,0);(3.75,0);(6.25,0);(6.25,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\lugt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(21.25,25);(21.25,25);(21.25,8.75);(21.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(21.25,8.75);(21.25,8.75);(17.5,5);(17.5,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,5);(15,5);(15,2.5);(15,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,2.5);(15,2.5);(17.5,2.5);(17.5,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,5);(15,5);(17.5,5);(17.5,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,2.5);(17.5,2.5);(17.5,5);(17.5,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,17.5);(47.5,17.5);(48.75,16.25);(48.75,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(48.75,8.75);(48.75,8.75);(45,5);(45,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(48.75,11.25);(48.75,11.25);(48.75,8.75);(48.75,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(48.75,8.75);(48.75,8.75);(51.25,8.75);(51.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(48.75,11.25);(48.75,11.25);(51.25,11.25);(51.25,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(51.25,8.75);(51.25,8.75);(51.25,11.25);(51.25,11.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pregr$
%</text>
%<multicurve fill-style= "none"
%	 points= "(45,5);(45,5);(45,2.5);(45,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(46.25,2.5);(46.25,2.5);(46.25,0);(46.25,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(43.75,2.5);(43.75,2.5);(43.75,0);(43.75,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(43.75,2.5);(43.75,2.5);(46.25,2.5);(46.25,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(43.75,0);(43.75,0);(46.25,0);(46.25,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\lugt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(55,25);(55,25);(55,20);(55,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,20);(55,20);(51.25,16.25);(51.25,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(48.75,16.25);(48.75,16.25);(48.75,13.75);(48.75,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(48.75,13.75);(48.75,13.75);(51.25,13.75);(51.25,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(48.75,16.25);(48.75,16.25);(51.25,16.25);(51.25,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(51.25,13.75);(51.25,13.75);(51.25,16.25);(51.25,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,20);(47.5,20);(47.5,17.5);(47.5,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,17.5);(45,17.5);(47.5,17.5);(47.5,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,20);(45,20);(47.5,20);(47.5,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(46.25,18.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prunt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(45,20);(45,20);(45,17.5);(45,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,13.75);(50,13.75);(50,11.25);(50,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(51.25,8.75);(51.25,8.75);(55,5);(55,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,5);(55,5);(55,0);(55,0)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(55,25)
\psline(11.25,15)(11.25,12.5)
\psline(8.75,12.5)(11.25,12.5)
\psline(8.75,15)(11.25,15)
\rput(10,13.75){$\prunt$}
\psline(8.75,15)(8.75,12.5)
\psline(11.25,8.75)(15,5)
\psline(8.75,8.75)(5,5)
\psline(16.25,2.5)(16.25,0)
\psline(10,12.5)(10,11.25)
\psline(8.75,11.25)(8.75,8.75)
\psline(8.75,8.75)(11.25,8.75)
\psline(8.75,11.25)(11.25,11.25)
\psline(11.25,8.75)(11.25,11.25)
\rput(10,10){$\pregr$}
\psline(5,5)(5,2.5)
\psline(6.25,2.5)(6.25,0)
\psline(3.75,2.5)(3.75,0)
\psline(3.75,2.5)(6.25,2.5)
\psline(3.75,0)(6.25,0)
\rput(5,1.25){$\lugt$}
\psline(21.25,25)(21.25,8.75)
\psline(21.25,8.75)(17.5,5)
\psline(15,5)(15,2.5)
\psline(15,2.5)(17.5,2.5)
\psline(15,5)(17.5,5)
\psline(17.5,2.5)(17.5,5)
\psline(47.5,17.5)(48.75,16.25)
\psline(48.75,8.75)(45,5)
\psline(48.75,11.25)(48.75,8.75)
\psline(48.75,8.75)(51.25,8.75)
\psline(48.75,11.25)(51.25,11.25)
\psline(51.25,8.75)(51.25,11.25)
\rput(50,10){$\pregr$}
\psline(45,5)(45,2.5)
\psline(46.25,2.5)(46.25,0)
\psline(43.75,2.5)(43.75,0)
\psline(43.75,2.5)(46.25,2.5)
\psline(43.75,0)(46.25,0)
\rput(45,1.25){$\lugt$}
\psline(55,25)(55,20)
\psline(55,20)(51.25,16.25)
\psline(48.75,16.25)(48.75,13.75)
\psline(48.75,13.75)(51.25,13.75)
\psline(48.75,16.25)(51.25,16.25)
\psline(51.25,13.75)(51.25,16.25)
\psline(47.5,20)(47.5,17.5)
\psline(45,17.5)(47.5,17.5)
\psline(45,20)(47.5,20)
\rput(46.25,18.75){$\prunt$}
\psline(45,20)(45,17.5)
\psline(50,13.75)(50,11.25)
\psline(51.25,8.75)(55,5)
\psline(55,5)(55,0)
\end{pspicture}


==> PIC/residues.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Apr 29 13:51:27 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="3.75" x-max="71.25" y-min="0" y-max="25" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(11.25,20);(11.25,20);(11.25,17.5);(11.25,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.75,17.5);(8.75,17.5);(11.25,17.5);(11.25,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.75,20);(8.75,20);(11.25,20);(11.25,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,18.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prunt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(8.75,20);(8.75,20);(8.75,17.5);(8.75,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,12.5);(11.25,12.5);(15,8.75);(15,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.75,12.5);(8.75,12.5);(5,8.75);(5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,8.75);(15,8.75);(15,0);(15,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,17.5);(10,17.5);(10,15);(10,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.75,15);(8.75,15);(8.75,12.5);(8.75,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.75,12.5);(8.75,12.5);(11.25,12.5);(11.25,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.75,15);(8.75,15);(11.25,15);(11.25,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,12.5);(11.25,12.5);(11.25,15);(11.25,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pregr$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,8.75);(5,8.75);(5,6.25);(5,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.25,6.25);(6.25,6.25);(6.25,3.75);(6.25,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,6.25);(3.75,6.25);(3.75,3.75);(3.75,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,6.25);(3.75,6.25);(6.25,6.25);(6.25,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,3.75);(3.75,3.75);(6.25,3.75);(6.25,3.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\lugt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xil$
%</text>
%<multicurve fill-style= "none"
%	 points= "(66.25,20);(66.25,20);(66.25,17.5);(66.25,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(63.75,17.5);(63.75,17.5);(66.25,17.5);(66.25,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(63.75,20);(63.75,20);(66.25,20);(66.25,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,18.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prunt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(63.75,20);(63.75,20);(63.75,17.5);(63.75,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(66.25,12.5);(66.25,12.5);(70,8.75);(70,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(63.75,12.5);(63.75,12.5);(60,8.75);(60,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,8.75);(60,8.75);(60,0);(60,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,17.5);(65,17.5);(65,15);(65,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(63.75,15);(63.75,15);(63.75,12.5);(63.75,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(63.75,12.5);(63.75,12.5);(66.25,12.5);(66.25,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(63.75,15);(63.75,15);(66.25,15);(66.25,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(66.25,12.5);(66.25,12.5);(66.25,15);(66.25,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pregr$
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,8.75);(70,8.75);(70,6.25);(70,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(71.25,6.25);(71.25,6.25);(71.25,3.75);(71.25,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(68.75,6.25);(68.75,6.25);(68.75,3.75);(68.75,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(68.75,6.25);(68.75,6.25);(71.25,6.25);(71.25,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(68.75,3.75);(68.75,3.75);(71.25,3.75);(71.25,3.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xir$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\rugt$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(71.25,25)
\psline(11.25,20)(11.25,17.5)
\psline(8.75,17.5)(11.25,17.5)
\psline(8.75,20)(11.25,20)
\rput(10,18.75){$\prunt$}
\psline(8.75,20)(8.75,17.5)
\psline(11.25,12.5)(15,8.75)
\psline(8.75,12.5)(5,8.75)
\psline(15,8.75)(15,0)
\psline(10,17.5)(10,15)
\psline(8.75,15)(8.75,12.5)
\psline(8.75,12.5)(11.25,12.5)
\psline(8.75,15)(11.25,15)
\psline(11.25,12.5)(11.25,15)
\rput(10,13.75){$\pregr$}
\psline(5,8.75)(5,6.25)
\psline(6.25,6.25)(6.25,3.75)
\psline(3.75,6.25)(3.75,3.75)
\psline(3.75,6.25)(6.25,6.25)
\psline(3.75,3.75)(6.25,3.75)
\rput(5,5){$\lugt$}
\rput(10,25){$\xil$}
\psline(66.25,20)(66.25,17.5)
\psline(63.75,17.5)(66.25,17.5)
\psline(63.75,20)(66.25,20)
\rput(65,18.75){$\prunt$}
\psline(63.75,20)(63.75,17.5)
\psline(66.25,12.5)(70,8.75)
\psline(63.75,12.5)(60,8.75)
\psline(60,8.75)(60,0)
\psline(65,17.5)(65,15)
\psline(63.75,15)(63.75,12.5)
\psline(63.75,12.5)(66.25,12.5)
\psline(63.75,15)(66.25,15)
\psline(66.25,12.5)(66.25,15)
\rput(65,13.75){$\pregr$}
\psline(70,8.75)(70,6.25)
\psline(71.25,6.25)(71.25,3.75)
\psline(68.75,6.25)(68.75,3.75)
\psline(68.75,6.25)(71.25,6.25)
\psline(68.75,3.75)(71.25,3.75)
\rput(65,25){$\xir$}
\rput(70,5){$\rugt$}
\end{pspicture}

